Ftklipse - Design and Implementation of an Extendable Computer Forensics Environment: Software Requirements Specification Document

The purpose behind this article is to describe the features of Ftklipse, an extendable platform for computer forensics. This document designed to provide a detailed specification for the developers of Ftklipse. Ftklipse is a thick-client solution for forensics investigation. It is designed to collect and preserve evidence, to analyze it and to report on it. It supports chain of custody management, access control policies, and batch operation of its included tools in order to facilitate and accelerate the investigation. The environment itself and its tools are configurable as well and is based on Eclipse.

==> conclusion.tex <==
\chapter{Conclusions}

$Revision: 1.1 $

\section{Acknowledgments}
We would like to thank Dr. Debbabi for allowing this project in the context
of his INSE 6150 course.
%{\todo}

% EOF


==> date.tex <==
Sat 13 Jun 2009 00:45:48 EDT


==> methodology.tex <==
\chapter{Methodology}

$Revision: 1.1 $

{\todo}

% EOF


==> toc.tex <==
\pagenumbering{roman}
\tableofcontents
\clearpage
\pagenumbering{arabic}

%\listoffigures
%\listoftables

